Uniform Distribution Technique for Neutrino Beam Scan Simulation

In Fermilab's neutrino facilities such as the Neutrinos at the Main Injector (NuMI) and the upcoming Long Baseline Neutrino Facility (LBNF), a proton beam strikes high-power target, producing positively and negatively charged pions and kaons. There is a need for detailed simulations in order to capture all particle interactions and beam propagation from protons on target to short-lived mesons decaying into muons and neutrinos. The generation of individual beam simulations is a resource-intensive and time-consuming process. In this paper, we describe a method through which many simulation samples with high statistics can be generated to study the effects of beam scan across a target for given beam configurations.

==> NuMIMuonMonitors.tex <==
\section{NuMI muon monitors}
There are three beam monitors in the NuMI beam line after the absorber called muon monitors, separated by 12 and 18 m of rock, making them sensitive to muons of different momenta. In the absorber volume, most particles generated upstream of the absorber are removed except for muons. The muons are detected at the muon monitors. When muons reach these muon monitors, they lose energy through processes known as ionization energy loss. Each muon monitor consists of a $9×9$ array of ionization chambers as shown in Fig.~\ref{fig:MM}. There are two parallel plate electrodes separated by a 3-mm gap in each ionization chamber filled which is filled with He gas. 
\begin{figure}[htpb!]
  \begin{center}\setlength{\unitlength}{1.0cm}
   \includegraphics[width=.4\textwidth]{AllNewPlots/MM.png}
\caption{Schematics of the NuMI muon monitors.}\label{fig:MM}
    \end{center}
  \end{figure}
